From Narrative to Auditable Forecasts: A Structured Scaffold for Agentic Forecasting

LLM agents are increasingly used for live forecasting, where they retrieve up-to-date information and produce estimates for unresolved future events. However, current agentic forecasting often relies on implicit narrative aggregation: agents collect evidence, discuss it in prose, and often assign a probability without an explicit update path from evidence to forecast. This limits both forecasting accuracy and auditability. We propose AuditForecast, an agentic scaffold for structured probabilistic forecasting. AuditForecast first anchors the forecast with a suitable quantitative baseline model, uses model-guided data retrieval to derive a base probability, and then applies situational factor updates outside the model's scope through mechanical aggregation in odds space. This turns forecasting from a prose-based judgment into a structured process with explicit intermediate objects. Across multiple live forecasting benchmarks, AuditForecast improves forecasting accuracy and calibration relative to strong agentic baselines, surpasses market-implied references in several settings, and outperforms substantially more expensive deep-research agents while remaining Pareto-dominant in the cost--accuracy tradeoff. Beyond performance gains, AuditForecast produces an auditable forecasting report that makes forecast construction explicit and supports systematic post hoc analysis.

==> Sections/ethical.tex <==
\section*{Ethical Considerations}
This work is dedicated to investigating the security and safety vulnerabilities associated with opinion editing in Large Language Models. Our goal is to deepen understanding of how factual opinions, meaning verifiable stances of public figures on major social and political issues, can be maliciously manipulated through existing editing techniques. By systematically studying these vulnerabilities, we aim to raise awareness of potential risks and support the development of more robust defense mechanisms. When releasing our benchmark and related resources, we will provide detailed usage guidelines that specify responsible use cases and restrictions, explicitly prohibiting any application for misinformation generation or character defamation. All factual opinions are derived from publicly verifiable sources, and counterfactual edits are constructed solely for controlled evaluation purposes. We emphasize that the proposed methods and analyses are intended exclusively for advancing research on LLM safety, transparency, and robustness. By revealing potential vulnerabilities in factual opinion editing, we hope to foster a more comprehensive understanding of the associated security risks and to contribute to the responsible development and deployment of LLMs in real-world settings.

\section*{Acknowledgements}
We thank the anonymous reviewers for their valuable feedback. The authors acknowledge the National Artificial Intelligence Research Resource (NAIRR) Pilot for contributing to this research result. The work is partially supported by the
National Science Foundation under Grant No.2450546. The views and conclusions contained in this paper are those of the authors and should not be interpreted as representing any funding agencies.

==> Sections/limitations.tex <==
\section*{Limitations}
While our study provides a comprehensive analysis of factual opinion editing and its associated risks, several limitations remain to be addressed in future research. First, our current experiments are conducted under a single-editing setting. The results already reveal noticeable overfitting issues, as reflected by degraded locality performance. Extending the framework to multi-editing scenarios, such as simultaneously modifying multiple issues associated with the same public figure, would present greater challenges and serve as an important direction for future investigation.

Second, this work primarily focuses on exposing and understanding the potential security vulnerabilities of opinion editing, while a systematic exploration of corresponding defense mechanisms remains limited. We outline several promising directions for defense development. Although the edited models can generate seemingly plausible supporting evidence, much of this content is fabricated. Therefore, fact-checking such evidence, for example by retrieving and verifying external information through retrieval-augmented generation (RAG) systems or by validating the existence of the claimed evidence sources, could help detect traces of manipulation. In addition, the severe overfitting behaviors observed after editing might also serve as detectable signals. We hope that our benchmark will encourage the research community to further investigate and develop robust defense mechanisms against such opinion-level manipulations.
